Maximising information from weak lensing galaxy surveys

Weak lensing galaxy surveys are currently undergoing a dramatic revolution as the dawn of the Stage-IV surveys are upon us. Hence, ensuring that our analysis methods are as accurate and precise as the raw data is of upmost importance. This motivated the development of a new implementation of the quadratic maximum likelihood power spectrum estimation technique, the application of the theoretical uncertainties approach to mitigate baryonic feedback biases, and to re-evaluating the criterion from which binary scale cuts are derived when aiming to eliminate baryonic biases. These techniques maximise the available information from weak lensing observations while minimising potential systematic biases, and shows how this PhD thesis contributes to the advancement of weak lensing cosmology.

==> chapters/declaration.tex <==

I declare that this thesis was written by myself, that the work contained herein
is my own, except where explicitly stated otherwise by citation or acknowledgment
in the text, and that this thesis
has not been submitted for any other degree or professional qualification. 

In Chapters \ref{chp:introduction}, \ref{chp:background_cosmology}, 
\ref{chp:grav_lensing}, and \ref{chp:Cosmology_2024}, we present a review of
modern cosmology, with a detailed investigation into weak lensing and its
applications in modern cosmology. This lays out the groundwork and motivations
for the later chapters.  

Chapter \ref{chp:QML_estimator} is an investigation into the development of a
new quadratic maximum likelihood estimator applied to cosmic shear, has been
published in Work~\cite{Maraio:2022ywi}. 

Chapter \ref{chp:baryonic_effects} presents an investigation into applying the
theoretical error method to baryonic effects in the matter power spectrum and
its application to cosmic shear, and has been published in
Work~\cite{Maraio:2024xjz}.

Chapter~\ref{chp:binary_cuts} investigates an alternative method to mitigating
baryonic effects in cosmic shear through the use of binary scale cuts. 

Chapter~\ref{chp:conclusions} summarises the new work presented in this thesis,
with an outlook to the future.


\begin{flushright}
    \textit{Alessandro Maraio\\
     February 2025}
  \end{flushright}
